Inverse-problem versus principal component analysis methods for angular differential imaging of circumstellar disks. The mustard algorithm

Circumstellar disk images have highlighted a wide variety of morphological features. Recovering disk images from high-contrast angular differential imaging (ADI) sequences are however generally affected by geometrical biases, leading to unreliable inference of the morphology of extended disk features. Recently, two types of approaches have been proposed to recover more robust disk images from ADI sequences: iterative principal component analysis, and inverse problem approaches. We introduce MUSTARD, a new IP-based algorithm designed to address the problem of the flux invariant to the rotation in ADI sequences; a limitation inherent to the ADI observing strategy, and discuss the advantages of IP approaches with respect to PCA-based algorithms. The MUSTARD model relies on the addition of morphological priors on the disk and speckle field to a standard IP approach to tackle rotation-invariant signal in circumstellar disk images. We compare the performance of MUSTARD, I-PCA, and standard PCA on a sample of high-contrast imaging data sets acquired in different observing conditions, after injecting a variety of synthetic disk models at different contrast levels. MUSTARD significantly improves the recovery of rotation-invariant signal in disk images, especially for data sets obtained in good observing conditions. However, the MUSTARD model is shown to inadequately handle unstable ADI data sets, and to provide shallower detection limits than PCA-based approaches. MUSTARD has the potential to deliver more robust disk images by introducing a prior to address the inherent ambiguity of ADI observations. However, the effectiveness of the prior is partly hindered by our limited knowledge of the morphological and temporal properties of the stellar speckle halo. In light of this limitation, we suggest that the algorithm could be improved by enforcing a prior based on a library of reference stars

==> bin.tex <==
Although \texttt{MAYONNAISE} can produce good-looking results, this approach lacks statistical validity. 

\subsection{Mask suboptimally}
\sj{THIS IS UNDER CONSTRCUTION. IT IS A NEW PROPOSITION, THIS IS NOT ERROR FREE.}

\sj{This Paragraph about the mask will be moved here if you like the propose section}
To sort out these ambiguities, we will have to use prior knowledge, for this purpose we added a prior on the morphology of the stellar halo. $M_{\mathrm{reg}}$ is a Gaussian, which represents the way the stellar halo spreads over the frame. Hence, this regularization will penalize certain flux distributions of ambiguous signals according to the shape of the mask. $M_{\mathrm{reg}}$ is defined as a Gaussian, with a width set to match the spread of the stellar halo. This regularization penalizes the flux distribution of ambiguous signals according to the shape of the mask. While fine-tuning of the mask from a dataset to another is expected to improve our results, we rather considered a realistic case scenario of not knowing beforehand the stellar halo profile due to the potential presence of bright disk signals. We therefore considered manually a single Gaussian profile matching the expected amount of rotation-invariant flux based on the radial profile of the stellar halo. This led to satisfying results in most cases. Although, a more complex mask (e.g., learned from a library of PSFs) could be used (see \ref{sec:discussion}).

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{Images/mask_subopt.png}
    \caption{ADI cube and Gaussian approximation}
    \label{fig:mask_subpot}
\end{figure}

\sj{In addition some more texte to talk about the figure.}
In the absence of a reliable model, or reference star, we have to build our own prior to reconstruct the correct PSF, respecting flux ambiguous to the rotation. In the Fig~\ref{fig:mask_subpot}, we show that removing a Gaussian-like shapes could help to have an idea of what the disk would look like without flux invariant to the rotation. In this example, with computed a mask using the empty cube before disk injection. Obviously, this cannot be done with real observation, which is why the choice of the mask is a critical point. When fitting a Gaussian over a dataset containing the disk, some disk signal will fall into the Gaussian. Nevertheless, this can still be used if needed. This will broadly reduce the flux invariant to the rotation. Without fitting the mask but rather used it as a regularization to fit, we avoid partially that the inaccuracy of the mask fit.

With a classical PSF subtraction (or any other methods that do not preserve flux ambiguous to the rotation), we observe that there is a large amount of flux missing in the disk estimation. On the contrary, noADI consisting of averaging the derotated cube, we observe that there is too much flux. and fine structure might be drowned in stellar residual. Subtraction of the optimal Gaussian mask is one approximation which is not perfect, but could give an idea of what the disk could look-like without flux ambiguous to the rotation missing. \texttt{MUSTARD} propose an in-between, adding the prior as regularization, while it will be compensated by the smoothness regularization and the data-attachment term leveraging angular diversity.

\sj{END OF THE DANGER ZONE}
